General Lotto Games with Scouts: Information versus Strength

We introduce General Lotto games with Scouts: a General Lotto game with asymmetric information. There are two players, Red and Blue, who both allocate resources to a field. However, scouting capabilities afford Blue to gain information, with some probability, on the number of Red's resources before allocating his own. We derive optimal strategies for this game in the case of a single field. In addition we provide upper and lower bounds of the value of the game in a multi-stage case with multiple battlefields. We devise several ways to characterise the influence of information versus strength. We conclude by drawing qualitative insights from these characterisations and the game values, and draw parallels with military practice.

==> abstract.tex <==

%\tableofcontents

\section*{Abstract}
We introduce General Lotto games with Scouts: a two-stage General Lotto game with asymmetric information. There are two players, Red and Blue, who both allocate troops to a field. However, scouting capabilities afford Blue to gain information, with some probability, on the number of Red's troops before allocating his own. We derive optimal strategies for this game in the case of a single field. In addition we provide upper and lower bounds of the value of the game in a multi-stage case with multiple battlefields.
%These bounds are tight in some settings.
We devise several ways to characterise the value of information versus strength. We conclude by drawing qualitative insights from these characterisations and the game values, and draw parallels with military practice. 

==> packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath,amsthm,mathrsfs}
\usepackage{amsfonts}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{adjustbox}

\usepackage[title]{appendix}%
\usepackage{textcomp}%
\usepackage{manyfoot}%
\usepackage{booktabs}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage[obeyFinal,textsize=footnotesize]{todonotes}

\usepackage[comma, sort&compress, authoryear]{natbib} %For bibliography
\usepackage{hyperref}% This is for hyperlinks
\hypersetup{ colorlinks=true, linkcolor=blue, citecolor=blue,
  filecolor=blue, urlcolor=blue}

%custom settings
\setlength\parindent{0pt}

%custom commands
\newcommand{\1}{\mathbbm{1}}
\newcommand{\Bin}{\mathrm{Bin}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\p}{\mathbb{P}}

\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
